Neural Finite-State Machines for Surgical Phase Recognition

Surgical phase recognition (SPR) is crucial for applications in workflow optimization, performance evaluation, and real-time intervention guidance. However, current deep learning models often struggle with fragmented predictions, failing to capture the sequential nature of surgical workflows. We propose the Neural Finite-State Machine (NFSM), a novel approach that enforces temporal coherence by integrating classical state-transition priors with modern neural networks. NFSM leverages learnable global state embeddings as unique phase identifiers and dynamic transition tables to model phase-to-phase progressions. Additionally, a future phase forecasting mechanism employs repeated frame padding to anticipate upcoming transitions. Implemented as a plug-and-play module, NFSM can be integrated into existing SPR pipelines without changing their core architectures. We demonstrate state-of-the-art performance across multiple benchmarks, including a significant improvement on the BernBypass70 dataset - raising video-level accuracy by 0.9 points and phase-level precision, recall, F1-score, and mAP by 3.8, 3.1, 3.3, and 4.1, respectively. Ablation studies confirm each component's effectiveness and the module's adaptability to various architectures. By unifying finite-state principles with deep learning, NFSM offers a robust path toward consistent, long-term surgical video analysis.

==> sections/2_related_work.tex <==
\section{Related Work}
\label{section:related_work}

% \subsection{Surgical Phase Recognition}
\noindent{\bf{Deep Learning Models.}} The evolution of surgical phase recognition has been marked by increasingly sophisticated neural architectures. EndoNet~\cite{TwinandaSMMMP17endonet} pioneered CNN-based feature extraction with hierarchical hidden Markov models for temporal modeling. MTRCNet-CL~\cite{JinLDCQFH20mrcnet} advanced this by correlating tool presence with surgical phases, though requiring additional annotations.
LSTM-based approaches~\cite{JinD0YQFH18sv-rcnet,YiJ19hfom,GaoJDH20treesearch} successfully integrated spatial-temporal information, but faced vanishing gradient issues with lengthy surgical videos. To address this, TMRNet~\cite{JinLCZDH21tmrnet} introduced non-local bank operators, while TeCNO~\cite{czempiel2020tecno} employed temporal convolutional networks~\cite{LeaVRH16tcn,FarhaG19mctcn} for long-term temporal modeling.
The advent of transformers~\cite{VaswaniSPUJGKP17transfomer} and ViT~\cite{DosovitskiyB0WZ21vit} enabled parallel processing of longer sequences. This led to various architectures: TAPIR~\cite{valderrama2020tapir} with MViT~\cite{FanXMLYMF21mvit}, Trans-SVNet~\cite{GaoJLDH21transsvnet} combining transformers with TCNs, and Surgformer~\cite{yang2024surgformer} introducing Hierarchical Temporal Attention. Pelphix~\cite{KilleenZMATOU23_Pelphix} adapted transformers for X-ray phase prediction, while Ding et al.~\cite{ding2024towards} enhanced Surgformer's robustness through digital twin representation. LoViT~\cite{Liu23Lovit} employs informer~\cite{ZhouZPZLXZ21informer} for memory-efficient encoding, while SKiT~\cite{liu2023skit} introduces key-reordering with temporal max-pooling. While these approaches advance architectural efficiency, our NFSM takes an orthogonal approach by incorporating transition learning to develop procedural understanding.

\noindent{\bf{Hidden Markov Models.}} Before the deep learning era, surgical phase recognition primarily relied on statistical models, particularly hidden Markov models (HMMs)~\cite{BlumPFN08HMM,BhatiaOXH07RL_video_hmm,CadeneRTC16CNN_HMM_SMOOTHING,PadoyBFBN08_online,BlumFN10,PadoyBAFBN12,DergachyovaBHMJ16}. These approaches modeled surgical procedures as finite-state machines, defining transitions between predefined states and their observations.
Early methods faced challenges with visual feature extraction. Padoy et al.\cite{PadoyBFBN08_online} relied on hand-crafted features like hue histograms and tool-specific colors, while Blum et al.\cite{BlumFN10} employed canonical correlation analysis to correlate visual features with manual annotations. Dergachyova et al.~\cite{DergachyovaBHMJ16} advanced this through ensemble AdaBoost classifiers for phase distinction based on visual features. Many approaches~\cite{BlumFN10,PadoyBAFBN12,BardramDJLNP11,HoldenUSMCGPF14,PadoyBFBN08_online} required supplementary information from instrument annotations or additional sensors, with transition probabilities typically derived through statistical methods~\cite{PadoyBFBN08_online,BlumFN10,DergachyovaBHMJ16}. In contrast to these static, statistically-derived transitions, our NFSM learns dynamic transition tables specific to each input sequence, while leveraging powerful deep learning features instead of hand-crafted ones.

% \subsection{Neural State Machine}
% There are some attempts to model the state machine concept in neural network form. Hudson \textit{et al.}~\cite{hudson_neural_state_machine} use the state machine to represent semantic components of the image features and enable reasoning via state transition among the semantic components. Starke \textit{et al.}~\cite{Starke_neural_state_machine_iteraction} proposed a neural state machine to enhance character-scene interactions in a data-driven way in computer graphics. Johnson \textit{et al.}~\cite{Johnson_finite_state_automation} introduced a finite-state automaton layer to learn the graph structure in the graph-based neural network model. Although the finite state machine concept achieved success in those areas, its neural instantiation has not been explored in video analysis. To our knowledge, our work is the first to incorporate the finite-state machine concept as a neural module for video analysis.


